Variable Impedance Control in End-Effector Space: An Action Space for Reinforcement Learning in Contact-Rich Tasks

Reinforcement Learning (RL) of contact-rich manipulation tasks has yielded impressive results in recent years. While many studies in RL focus on varying the observation space or reward model, few efforts focused on the choice of action space (e.g. joint or end-effector space, position, velocity, etc.). However, studies in robot motion control indicate that choosing an action space that conforms to the characteristics of the task can simplify exploration and improve robustness to disturbances. This paper studies the effect of different action spaces in deep RL and advocates for Variable Impedance Control in End-effector Space (VICES) as an advantageous action space for constrained and contact-rich tasks. We evaluate multiple action spaces on three prototypical manipulation tasks: Path Following (task with no contact), Door Opening (task with kinematic constraints), and Surface Wiping (task with continuous contact). We show that VICES improves sample efficiency, maintains low energy consumption, and ensures safety across all three experimental setups. Further, RL policies learned with VICES can transfer across different robot models in simulation, and from simulation to real for the same robot. Further information is available at https://stanfordvl.github.io/vices.

==> legacy/1_intro-bak.tex <==
% -----------
%
%Present the problem
In reinforcement learning (RL) an agent explores the environment through actions in order to achieve a task. The goal is to learn a mapping between observations of the environment to the optimal next best action. While the community has extensively studied how different representations of the observation space influence the learning process, much less effort has been applied to understand the consequences of different action spaces in the learning process and resulting behavior.

Nowadays, most robotic platforms~\cite{} are equipped with a set of controllers that differ in the action space. Some send joint space commands (e.g. position, velocity or torque) or task space commands (e.g. endeffector poses or impedance). This allows roboticists to freely select the most suitable action space for a particular application. \jean{I think this is not only picked by intuition in RL but also just in robot motion control} However, picking the right action space for a reinforcement learning problem is still an uninformed process guided by a hunch or, in the best cases, from previous experience, 
\jean{it is kind of guided by the characteristics of the problem though ... but maybe not formally analyzed. Most people pick the controller that closes the loop around the quantity they care about.}
instead of being guided by the characteristics of the problem. Nevertheless, the selection of the action space greatly impacts RL to the point of deciding if the agent can solve the task or not~\cite{Peng:2017:LLS:3099564.3099567}.

\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figures/f1.pdf}
\caption{Depending the characteristics of the task, different action spaces for policy learning are best suited than others. Variable impedance in task space is efficient for agents to learn to contact-rich tasks and can be also applied to contact-free. Through the compensation of the robot's kinematics and dynamics the policies learned for one robot in simulation transfer seamlessly to other robot instances and to the real robot}
\label{fig1}
\end{figure}

% First contribution: evaluation of action spaces
\jean{This paper presents an empirical study of the different action spaces for RL when learning contact rich manipulation tasks}
Our goal in this paper is twofold: first, we aim to understand the benefits and drawbacks of the most common action spaces in reinforcement learning when applied to manipulation tasks involving different amount of contact. We evaluate different actions spaces in terms of learning efficiency, physical efficiency (i.e. energy consumption), generality between task instances, and transferability between robots.
\jean{some funny words above. With learning efficiency do you mean whether a certain reward is reached at all or how much data is needed to reach a certain level of accuracy. I would also write about generalization in both cases, to tasks and robots or talk about transfer to both cases.}

% Second contribution: new action space. Motivation: Why is dynamic impedance Cartesian trajectories a good idea
\jean{is it a novel action space though? Has been used before.} \jean{paragraph needs smoothing and crispness but makes the rights points.}
Second, we propose and evaluate a novel action space suited to learn contact-rich interaction policies: variable impedance in Cartesian space. 
Impedance control allows contact rich manipulation tasks with uncertain environments by balancing the transfer between error in desired position and amount of force applied to the environment.
Compared to only-kinematics action spaces (i.e. position control), impedance control is safer and best suited to tasks. On the other hand, compared to joint space, Cartesian space is most intimately related to the manipulation task.

We evaluate the most common action spaces and compare them to our proposed action space in three prototypical robotic tasks: free space motion through viapoints, door opening and surface wiping. These three tasks span different levels of contact with the environment. We show that our proposed action space is the most efficient/safe \todo{check} for tasks with rich contact dynamics. Moreover, we demonstrate that policies learned in simulation in dynamic impedance Cartesian space transfer seamlessly between different robots, thanks to the task-closer nature of the space. And we also show that a classical operational space formalism~\cite{khatib1987unified} allows to transfer the policy learned in simulation to a real robot, even when the observation space is high-dimensional images, both in real and in simulation.
\jean{mention sim and real experiments. Mention visual input as well for wiping or at least high-dimensional one}


==> legacy/1_intro-v2.tex <==
\section{Introduction}
\label{sec:intro}
% \jean{still not so hot about the first paragraph ... it just doesn't connect to what comes next. It hints at redundancy but from the second paragraph this doesn't seem to come up. Do we need to talk about humans? Should we rather talk about the robot examples here and move these forward? I'm referring to the ones that close the loop around specific quantities.}
% For humans, the simple act of wiping a table clean is highly redundant with a multiplicity of solutions in the space of muscle actuation. Nevertheless, humans perform these contact-rich tasks effortlessly: we decide which part to wipe next and coordinate our muscles to execute the motion. It has been a challenge to perform such seemingly simple tasks with a robot such that it generalizes to a variety of scenarios, e.g. with different material properties. 


The motion control system of a robot is usually structured into at least two stages, or feedback control loops: an outer loop controller that generates some reference trajectory, and an inner loop controller that tracks this trajectory. Let us refer to the outer loop as a functional map from observations to reference signals $g(o): \mathcal{O} \rightarrow \mathcal{A}$, and the inner loop as a map from reference signals to actuation commands $f(a): \mathcal{A} \rightarrow \mathcal{U}$. Hence the control law becomes: $u = f\circ g (o)$, where $o \in \mathcal{O}$ is some observation, $a \in \mathcal{A}$ is an abstract action providing a reference signal in some space and $u \in \mathcal{U}$ is the control command sent to the robot's actuators to track this reference. 
% This framework allows for different control frequencies between the inner and outer loop. 

While control theory provides a vast repertoire of map strategies from reference signals to actuation commands ($f(\cdot)$ implementations), a key problem in robotics is to generate a viable reference in a suitable space given raw sensory observations, i.e. modelling the function $g(\cdot)$ and deciding on the interface to $f(\cdot)$. Once the interface has been defined, the generation of reference signals has been addressed in multiple ways, ranging from hand-tuned state machines~\cite{sen2016automating,khansari2016adaptive,murali2015learning}, trajectory optimization~\cite{18-toussaint-RSS,2017_rss_system}, imitation learning~\cite{schaal2003computational,Ijspeert:2013:DMP,Calinon08IROS,kroemer2015towards}, or reinforcement learning (RL)~\cite{lee2019making,harrison2017adapt}. This paper studies how the selection of an interface between $g(\cdot)$ and $f(\cdot)$ (the space $\mathcal{A}$) affects RL as method to learn the mapping from observations to reference signals $g(\cdot)$. 

Many recent RL studies focus on ``observations-to-torques''~\cite{levine2016end}, which is akin to merging $f(\cdot)$ and $g(\cdot)$ into a single learned model. 
Other methods use higher-level action spaces, such as joint space commands (e.g. position or velocity)~\cite{gu2017deep,haarnoja2018soft,vevcerik2017leveraging,zhu2018reinforcement} or task space commands (e.g. end-effector poses, force or impedance)~\cite{lee2019making,Mrinal:2011}. These works typically focus on the effects of choosing an observation space $\mathcal{O}$ on the learning process and rarely justify the choice of action spaces, $\mathcal{A}$. 
% However, we know from many examples in robot control that the choice of action space matters for task performance. 
However, the choice of action space defines around which quantity the inner control loop is closed and therefore in which space tracking error is minimized, critically impacting robustness and performance as well as exploration. 
For example, for walking robots it is important to directly control contact interactions to avoid slipping~\cite{Ludo_Contact_2013}. 
For a tennis swing, it is important to control and track a particular position, velocity and acceleration of the end-effector~\cite{DMP_Initial_2002}. 
For a surface-to-surface alignment task, minimizing the moment around a contact is important for robustness~\cite{khansari2016adaptive}. 

\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figures/f1b.pdf}
\caption{Depending on the characteristics of a task, different action spaces for policy learning are better suited than others; Variable impedance in end-effector space is efficient to learn contact-rich tasks and can be also applied to free-space motion; Through the compensation of the robot's kinematics and dynamics the policies learned for one robot in simulation transfer seamlessly to other robot instances and to the real robot}
\label{fig1}
\end{figure}

From this perspective, it makes sense that the choice of action space also impacts performance of RL training, with many action spaces not leading to convergence at all~\cite{Peng:2017:LLS:3099564.3099567}.
Intuitively, if the structure of the inner control loop $f(\cdot)$ is known, as is often the case with the kinematics and dynamics of robots consisting of multiple rigid bodies, then learning the function $g(\cdot)$ can be simplified. 
\jean{the below is the first time after many many sentences that you mention terms that have occurred in the abstract. I think this entire intro has to be restructured.}
In fact, studies in computational motor control confirm this hypothesis, stating that for a given robotic system, the system dynamics can be decoupled into robot dynamics and task space dynamics (lower-dimensional subspace relevant to task achievement)~\cite{mistry2015representation}. This decomposition enables planning and control of tasks in a simplified, reduced-dimensional space, while being robust to errors in robot and environment models.

This paper studies this decomposition for various choices of action spaces $\mathcal{A}$ and presents an empirical study comparing them for deep RL. The choice of action space should be guided not only by the robot model but also by prior knowledge of the task. Hence, we compare action spaces across tasks with varying degrees of task-space constraints, i.e., trajectory tracking with no contact, manipulation of constrained mechanisms, and continuous unconstrained contact.

Moreover, consider a contact-rich task such as wiping a board, wherein a robot must control forces in some directions (to keep pressing against the board) and motion in others. We hypothesize that an action space which captures motion and impedance in end-effector space can enable efficient learning for such tasks. The physical constraints of the task dictate in which axes the robot should be stiff and which should be compliant, and this can often be time-varying. Manual specification of the task constraints is not a scalable solution for the variety of contact-rich tasks the robot may need to perform. And even more, for some tasks, this specification may be non-intuitive. We address this by introducing \textit{Variable Impedance Control in End-Effector Space (VICES)} 
% \jean{this seems like a fairly common thing to do. Shoudl we really create 'our' acronym?} 
in a Deep Reinforcement Learning setting for contact-rich manipulation. 
We show that policies defined in end-effector space improve sample efficiency for exploration in RL, energy efficiency, and reduce peak forces. Furthermore, policies learned in end-effector space are robust to transfer across robots in simulation or the real world with significant difference in dynamics. Our primary contributions are:
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    leftmargin=*,
    itemindent=12pt]
\item An empirical study of performance of eight action space choices in deep RL comparing joint position, joint velocity, joint torque, joint variable impedance, end-effector fixed impedance, and end-effector variable impedance. The evaluation of these choices is performed on three prototypical robotic tasks: free space trajectory following, door opening, and surface wiping. These three tasks span different levels of task-space constraints and contact with the environment.
\item We show that policies learned in simulation with variable impedance in end-effector space best transfer between different robot models thanks to the task-closer nature of the space. Additionally, the classical dynamically consistent operational space formalism~\cite{khatib1987unified} allows us to transfer the policy learned in simulation to a real robot, even when the observation space is high-dimensional images, both in real and in simulation.
\end{enumerate}



==> legacy/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% % ----
% 1. RL can explore states spaces with varied reward models. However the choice of action space matters.
% 2. Particularly in robotics, where sample efficiency matters, this choice is even more important.
% 3. Additionally, depending on choice of action space, the problem may be either partially observed or underactuated.
% Eg for partial observation: position control for a contact task without force/torque feedback. State is position and so are actions.
% Eg. for underactuation: with joint torques (not impedance) the control dimension is much fewer which results in controlling a complicated dynamically evolving constraints.
% 3b. This limitation can result in both a penalty in sample complexity, and at times non-convergence.
% 4. This paper looks at variety of possible action spaces namely, …..{list}.
% 4b. We provide a continuum of tasks where we show that as complexity of implicit Task space constraints grows, the value of sophisticated action spaces becomes evident.
% 5. Further, among the chosen action spaces, we find that end effector impedance control performs the best and is transferable across robots in sim and from sim 2 real. While joint space impedance control can capture similar constraints as well owing to high degree of controllability. However, it implicitly also encodes the robot kinematics. This results in the model learning eccentricities of the simulation which may not be the same across different instance of the same robot, different kinematic structures or simulated and real robots.
% 6. We show our evaluation on three tasks — a. purely simulated task {X} to compare all action spaces, b. sim2sim transfer in task Y, and c. sim2real tranfer in task Z.


A simple motion of reaching for a cup is actually a highly-reduntant with a multiplicity of solutions in the space of muscle actuation. Nevertheless, humans perform these tasks effortlessly. Infact, studies in mammalian motion analysis show that agents control task-level quantities such as center-of-mass acceleration for balancing in cats~\cite{lockhart2007optimal}, and sit-to-stand movements in human~\cite{scholz1999uncontrolled}. In fact, studies in computational motor control  confirm this hypothesis through the minimum intervention principle, that is, motor output errors are only corrected when they interfere with task performance~\cite{todorov2002optimal}.

Yet, a majority of methods in reinforcement learning focus on ``percepts-to-torques''. The community has extensively studied how different representations of the observation space influence the learning process\tocite, and how variations in reward model can be handled to perform new tasks\tocite.
This has led to obviating the need for task specific observation models and meta-learning of task variations. However, the systematic evaluation of action spaces on learning efficiency and robustness has been lacking.  

Manipulation skill utilize task-space compliant control to achieve contact-rich manipulation to handle unmodeled disturbances due to the environment\tocite. In learning such tasks on real robots, efficiency and robustness becomes ever more important. Recent studies in learning based methods use a variety of action spaces varying from joint space commands (e.g. position, velocity or torque)\tocite or task space commands (e.g. endeffector poses or impedance)\tocite. Nevertheless, the action spce choice impacts performance of RL training, with many action models not converging at all~\cite{Peng:2017:LLS:3099564.3099567}.

It has been shown that for a given robotic system, the robot's dynamics can be decomposed into task-space (lower-dimensional subspace relevant to task achievement) and a null-space (orthogonal sub-space irrelevant to task). This decomposition enables planning and control of tasks in a simplified, reduced dimensional space, while still allowing for exploitation of redundancy for achieving secondary tasks or absorbing disturbances~\cite{mistry2015representation}. 
The choice of action space should be guided by prior knowledge of task and the complexity robot model and control. Yet, few studies justify their intuition formally, or provide comparative results.


\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figures/f1.pdf}
\caption{Depending the characteristics of the task, different action spaces for policy learning are best suited than others. Variable impedance in task space is efficient for agents to learn to contact-rich tasks and can be also applied to contact-free. Through the compensation of the robot's kinematics and dynamics the policies learned for one robot in simulation transfer seamlessly to other robot instances and to the real robot\ag{edit figure simulated images too dark!}}
\label{fig1}
\end{figure}

This paper presents an empirical study of different action spaces for deep reinforcement learning. These action spaces are compared across tasks with varying degrees of task-space constraints, i.e., trajectory tracking with no contact, intermittent contact and continuous contact. 
This is the first study to use \textit{Variable Impedance Control} in a Deep Reinforcement Learning setting for contact-rich manipulation. 
We show that when a dynamics model of the robot is approximately known, then actions controlling end-effector cartesian space are more sample efficient for exploration in RL, and energy efficient, and safe in peak forces. Further, policies learned with end-effector cartesian space actions are robust to transfer across robot dynamics in simulation and also facilitate simulation to real transfer.

\noindent Our primary contributions are:
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    leftmargin=*,
    itemindent=12pt]
\item An empirical study of performance of action space choice in deep RL comparing pose, velocity, force/torque control Joint Space and Enf-Effector Space. 
\item We evaluate the most common action spaces and compare them to our proposed action space in three prototypical robotic tasks: free space motion through viapoints, door opening and surface wiping. These three tasks span different levels of contact with the environment.
\item we demonstrate that policies learned in simulation in dynamic impedance Cartesian space transfer seamlessly between different robots, thanks to the task-closer nature of the space. And we also show that a classical operational space formalism~\cite{khatib1987unified} allows to transfer the policy learned in simulation to a real robot, even when the observation space is high-dimensional images, both in real and in simulation.
\end{enumerate}


\iffalse
----------- old stuff for comparison
%

%Present the problem
In reinforcement learning (RL) an agent explores the environment through actions in order to achieve a task. The goal is to learn a mapping between observations of the environment to the optimal next best action. While the community has extensively studied how different representations of the observation space influence the learning process, much less effort has been applied to understand the consequences of different action spaces in the learning process and resulting behavior.

Nowadays, most robotic platforms~\cite{} are equipped with a set of controllers that differ in the action space. Some send joint space commands (e.g. position, velocity or torque) or task space commands (e.g. endeffector poses or impedance). This allows roboticists to freely select the most suitable action space for a particular application. \jean{I think this is not only picked by intuition in RL but also just in robot motion control} However, picking the right action space for a reinforcement learning problem is still an uninformed process guided by a hunch or, in the best cases, from previous experience, 
\jean{it is kind of guided by the characteristics of the problem though ... but maybe not formally analyzed. Most people pick the controller that closes the loop around the quantity they care about.}
instead of being guided by the characteristics of the problem. Nevertheless, the selection of the action space greatly impacts RL to the point of deciding if the agent can solve the task or not~\cite{Peng:2017:LLS:3099564.3099567}.


% First contribution: evaluation of action spaces
\jean{This paper presents an empirical study of the different action spaces for RL when learning contact rich manipulation tasks}
Our goal in this paper is twofold: first, we aim to understand the benefits and drawbacks of the most common action spaces in reinforcement learning when applied to manipulation tasks involving different amount of contact. We evaluate different actions spaces in terms of learning efficiency, physical efficiency (i.e. energy consumption), generality between task instances, and transferability between robots.
\jean{some funny words above. With learning efficiency do you mean whether a certain reward is reached at all or how much data is needed to reach a certain level of accuracy. I would also write about generalization in both cases, to tasks and robots or talk about transfer to both cases.}

% Second contribution: new action space. Motivation: Why is dynamic impedance Cartesian trajectories a good idea
\jean{is it a novel action space though? Has been used before.} \jean{paragraph needs smoothing and crispness but makes the rights points.}
Second, we propose and evaluate a novel action space suited to learn contact-rich interaction policies: variable impedance in Cartesian space. 
Impedance control allows contact rich manipulation tasks with uncertain environments by balancing the transfer between error in desired position and amount of force applied to the environment.
Compared to only-kinematics action spaces (i.e. position control), impedance control is safer and best suited to tasks. On the other hand, compared to joint space, Cartesian space is most intimately related to the manipulation task.

We evaluate the most common action spaces and compare them to our proposed action space in three prototypical robotic tasks: free space motion through viapoints, door opening and surface wiping. These three tasks span different levels of contact with the environment. We show that our proposed action space is the most efficient/safe \todo{check} for tasks with rich contact dynamics. Moreover, we demonstrate that policies learned in simulation in dynamic impedance Cartesian space transfer seamlessly between different robots, thanks to the task-closer nature of the space. And we also show that a classical operational space formalism~\cite{khatib1987unified} allows to transfer the policy learned in simulation to a real robot, even when the observation space is high-dimensional images, both in real and in simulation.
\jean{mention sim and real experiments. Mention visual input as well for wiping or at least high-dimensional one}

\fi
